Scaling the Wild: Decentralizing Hogwild!-style Shared-memory SGD

Powered by the simplicity of lock-free asynchrony, Hogwilld! is a go-to approach to parallelize SGD over a shared-memory setting. Despite its popularity and concomitant extensions, such as PASSM+ wherein concurrent processes update a shared model with partitioned gradients, scaling it to decentralized workers has surprisingly been relatively unexplored. To our knowledge, there is no convergence theory of such methods, nor systematic numerical comparisons evaluating speed-up. In this paper, we propose an algorithm incorporating decentralized distributed memory computing architecture with each node running multiprocessing parallel shared-memory SGD itself. Our scheme is based on the following algorithmic tools and features: (a) asynchronous local gradient updates on the shared-memory of workers, (b) partial backpropagation, and (c) non-blocking in-place averaging of the local models. We prove that our method guarantees ergodic convergence rates for non-convex objectives. On the practical side, we show that the proposed method exhibits improved throughput and competitive accuracy for standard image classification benchmarks on the CIFAR-10, CIFAR-100, and Imagenet datasets. Our code is available at https://github.com/bapi/LPP-SGD.

==> results/Arch_res18_Data_imagenet.tex <==
\begin{tabular}{|>{\centering\arraybackslash}p{9.8mm}|>{\centering\arraybackslash}p{3.5mm}|>{\centering\arraybackslash}p{1.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.5mm}|}
\toprule
\textbf{Method} & $\mathbf{B}$ & $\mathbf{U}$ & \textbf{Tr.L.} & \textbf{Tr.A.} & \textbf{Te.L.} & \textbf{Te.A.} & $T$ \\
\midrule
\alsgd &       32 &             4 &     1.319 &      68.97 &    1.215 &     \textbf{70.58} &    \textbf{26237} \\
\palsgd &       32 &             4 &     1.397 &      68.31 &    1.257 &     69.91 &    24066 \\
\mbsgd &      128 &             - &     1.237 &      70.63 &    1.220 &     70.07 &    26772 \\
\mbsgd &       32 &             - &     1.339 &      68.53 &    1.231 &     70.13 &    30706 \\
\plsgd &      128 &             - &     1.256 &      70.22 &    1.223 &     70.02 &    25850 \\
\plsgd &       32 &             - &     1.350 &      68.32 &    1.236 &     70.02 &    31468 \\
\bottomrule
\end{tabular}

%\begin{tabular}{|>{\centering\arraybackslash}p{1.5mm}|>{\centering\arraybackslash}p{9.8mm}|>{\centering\arraybackslash}p{3.5mm}|>{\centering\arraybackslash}p{1.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.5mm}||}
%	\toprule
%	{} & \textbf{Method} & $\mathbf{B}$ & $\mathbf{U}$ & \textbf{Tr.L.} & \textbf{Tr.A.} & \textbf{Te.L.} & \textbf{Te.A.} & $T$ \\
%	\midrule
%	(1) &      \alsgd &       32 &             4 &     1.319 &      68.97 &    1.215 &     \textbf{70.58} &    \textbf{26237} \\
%	(2) &     \palsgd &       32 &             4 &     1.397 &      68.31 &    1.257 &     69.91 &    24066 \\
%	(3) &         \mbsgd &      128 &             - &     1.237 &      70.63 &    1.220 &     70.07 &    26772 \\
%	(4) &         \mbsgd &       32 &             - &     1.339 &      68.53 &    1.231 &     70.13 &    30706 \\
%	(5) &        \plsgd &      128 &             - &     1.256 &      70.22 &    1.223 &     70.02 &    25850 \\
%	(6) &        \plsgd &       32 &             - &     1.350 &      68.32 &    1.236 &     70.02 &    31468 \\
%	\bottomrule
%\end{tabular}



==> results/Arch_res50_Data_imagenet.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\toprule
\textbf{Method} & $B_{loc}$ & $U$ & \textbf{Tr.L.} & \textbf{Tr.A.} & \textbf{Te.L.} & \textbf{Te.A.} & $T$ \\
\midrule
\alsgd &       32 &             4 &     0.823 &      77.97 &    1.215 &     \textbf{76.58} &    54243 \\
\palsgd &       32 &             4 &     0.834 &      77.31 &    1.257 &     \textbf{76.11} &    \textbf{48066} \\
\mbsgd &      128 &             - &     0.809 &      78.63 &    1.220 &     76.07 &    52395 \\
\plsgd &      128 &             - &     0.818 &      78.22 &    1.223 &     76.12 &    50402 \\
\bottomrule
\end{tabular}


==> results/Arch_wnet168_Data_cifar10.tex <==
\begin{tabular}{llllll}
\toprule
{} & \textbf{Method} & $\mathbf{Q}$ & \textbf{Train{\newline}Acc.} & \textbf{Test{\newline}Acc.} & \textbf{Time{\newline}(S)} \\
\midrule
(1) &\alsgd &        2 &     100.00 &     94.92 &     6368 \\
(2) \palsgd &        2 &      99.97 &     94.89 &     5551 \\
(3) \mbsgd &        2 &     100.00 &     93.98 &     8265 \\
(4) \mbsgd &        2 &      95.68 &     88.42 &     7920 \\
(5) \plsgd &        2 &      99.99 &     94.21 &     8293 \\
(6) \plsgd &        2 &      95.34 &     88.33 &     7829 \\
(7) \alsgd &        4 &     100.00 &     94.91 &     3092 \\
(8) \palsgd &        4 &      99.96 &     94.87 &     2724 \\
(9) \mbsgd &        4 &     100.00 &     94.22 &     4045 \\
(10) \mbsgd &        4 &      99.87 &     89.46 &     3913 \\
(11) \plsgd &        4 &      99.98 &     94.02 &     4022 \\
(12) \plsgd &        4 &      98.52 &     84.45 &     3784 \\
(13) \alsgd &        8 &     100.00 &     94.69 &     1562 \\
(14) \palsgd &        8 &      99.99 &     93.78 &     1377 \\
(15) \mbsgd &        8 &     100.00 &     93.83 &     2116 \\
(16) \mbsgd &        8 &      87.54 &     73.97 &     2076 \\
(17) \plsgd &        8 &      99.98 &     94.18 &     2105 \\
(18) \plsgd &        8 &      89.19 &     81.80 &     1977 \\
\bottomrule
\end{tabular}
[6368,5551,8265,7920,8293,7829,3092,2724,4045,3913,4022,3784,1562,1377,2116,2076,2105,1977]

==> results/ArchsquuezenetDatacifar10.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}	
	\toprule
	\textbf{Method} & $B_{loc}$ & $U$ & \textbf{Tr.L.} & \textbf{Te.L.} & \textbf{Tr.A.} & \textbf{Te.A.} & \textbf{$T$}\\
	\midrule
	\alsgd &      128 &              4 &     0.004 &    0.385 &      \textbf{99.95} &     \textbf{92.48} &     \textbf{1251} \\ 
	\palsgd &      256 &               3 &     0.007 &    0.355 &      99.89 &     \textbf{92.55} &     \textbf{1027} \\ 
	\mbsgd &     1024 &       - &     0.003 &    0.325 &      99.97 &     91.50 &     1580 \\ 
	\mbsgd &      128 &               - &     0.005 &    0.294 &      99.93 &     92.41 &     2243\\
	\plsgd &     1024 &              - &     0.005 &    0.329 &      99.93 &     91.99 &     1202\\
	\plsgd &      128 &              - &     0.006 &    0.283 &      99.91 &     92.51 &     1843\\
	\bottomrule
\end{tabular} \caption{\small \sqn on \cft over the setting \textbf{S1}.}


%\begin{tabular}{||c|c|c|c|c|c|c|c||>{\centering\arraybackslash}p{9mm}|>{\centering\arraybackslash}p{3.5mm}|>{\centering\arraybackslash}p{1.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{3.5mm}||}	
%	\toprule
%	\textbf{Method} & $B_{loc}$ & $U$ & \textbf{Tr.L.} & \textbf{Te.L.} & \textbf{Tr.A.} & \textbf{Te.A.} & \textbf{$T$} & \textbf{Method} & $B_{loc}$ &  $U$ & \textbf{Tr.L.} & \textbf{Te.L.} & \textbf{Tr.A.} & \textbf{Te.A.} & \textbf{$T$}\\
%	\midrule
%\alsgd &      128 &              4 &     0.004 &    0.385 &      \textbf{99.95} &     \textbf{92.48} &     \textbf{1251} & \mbsgd &      128 &               - &     0.005 &    0.294 &      99.93 &     92.41 &     2243\\
%\palsgd &      256 &               3 &     0.007 &    0.355 &      99.89 &     \textbf{92.55} &     \textbf{1027} & \plsgd &     1024 &              - &     0.005 &    0.329 &      99.93 &     91.99 &     1202\\
% \mbsgd &     1024 &       - &     0.003 &    0.325 &      99.97 &     91.50 &     1580 & \plsgd &      128 &              - &     0.006 &    0.283 &      99.91 &     92.51 &     1843\\
%\bottomrule
%\end{tabular} \caption{\small Performance of \sqn on \cft over the setting \textbf{S1}.}


==> results/Archwnet168Datacifar100.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}	
	\toprule
	\textbf{Method} & $B_{loc}$ & $U$ & \textbf{Tr.L.} & \textbf{Te.L.} & \textbf{Tr.A.} & \textbf{Te.A.} & \textbf{$T$} \\
	\midrule
	\alsgd &       64 &            4 &     0.007 &    1.341 &      \textbf{99.98} &     \textbf{75.97} &     \textbf{1564} \\ 
	\palsgd &       64 &           3 &     0.008 &    1.554 &      \textbf{99.97} &     \textbf{75.42} &     \textbf{1376} \\ 
	\mbsgd &      128 &           - &     0.007 &    1.348 &      99.97 &     73.29 &     2115 \\ 
	\mbsgd &      512 &            - &     0.034 &    1.918 &      99.64 &     63.74 &     2076\\
	\plsgd &      128 &           - &     0.020 &    1.354 &     99.81 &     72.38 &      2108\\
	\plsgd &      512 &             - &     0.393 &    1.758 &      88.91 &     60.47 &     1976\\
	\bottomrule
\end{tabular} \caption{\small \wres-16x8 on \cfh over the setting \textbf{S3}.}
%\alsgd &       64 &          4 &     0.007 &    1.394 &      \textbf{99.98} &     \textbf{75.84} &     \textbf{1564} & \plsgd &      128 &           - &     0.023 &    1.354 &          2100\\
%\palsgd &       64 &          3 &     0.008 &    1.579 &      \textbf{99.98} &     \textbf{75.42} &     \textbf{1375} &  \plsgd &      512 &           - &     0.472 &    1.683 &      86.47 &     60.73 &     1971\\



%\begin{tabular}{||c|c|c|c|c|c|c|c||>{\centering\arraybackslash}p{9mm}|>{\centering\arraybackslash}p{3.5mm}|>{\centering\arraybackslash}p{1.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{4.0mm}|>{\centering\arraybackslash}p{3.5mm}||}	
%	\toprule
%	\textbf{Method} & $B_{loc}$ & $U$ & \textbf{Tr.L.} & \textbf{Te.L.} & \textbf{Tr.A.} & \textbf{Te.A.} & \textbf{$T$} & \textbf{Method} & $B_{loc}$ &  $U$ & \textbf{Tr.L.} & \textbf{Te.L.} & \textbf{Tr.A.} & \textbf{Te.A.} & \textbf{$T$}\\
%	\midrule
% \alsgd &       64 &            4 &     0.007 &    1.341 &      \textbf{99.98} &     \textbf{75.97} &     \textbf{1564} & \mbsgd &      512 &            - &     0.034 &    1.918 &      99.64 &     63.74 &     2076\\
%\palsgd &       64 &           3 &     0.008 &    1.554 &      \textbf{99.97} &     \textbf{75.42} &     \textbf{1376} & \plsgd &      128 &           - &     0.020 &    1.354 &     99.81 &     72.38 &      2108\\
%\mbsgd &      128 &           - &     0.007 &    1.348 &      99.97 &     73.29 &     2115 & \plsgd &      512 &             - &     0.393 &    1.758 &      88.91 &     60.47 &     1976\\
%\bottomrule
%\end{tabular} \caption{\small Performance of \wres-16x8 on \cfh over the setting \textbf{S3}.}
%%\alsgd &       64 &          4 &     0.007 &    1.394 &      \textbf{99.98} &     \textbf{75.84} &     \textbf{1564} & \plsgd &      128 &           - &     0.023 &    1.354 &          2100\\
%%\palsgd &       64 &          3 &     0.008 &    1.579 &      \textbf{99.98} &     \textbf{75.42} &     \textbf{1375} &  \plsgd &      512 &           - &     0.472 &    1.683 &      86.47 &     60.73 &     1971\\
%


==> results/res18/Arch_res18_Data_imagenet.tex <==
\begin{tabular}{lllllllll}
\toprule
{} & \textbf{Method} & $\mathbf{B}$ & $\mathbf{U}$ & \textbf{Tr.L.} & \textbf{Tr.A.} & \textbf{Te.L.} & \textbf{Te.A.} & $T$ \\
\midrule
(1) &      \alsgd &       32 &             4 &     1.319 &      68.97 &    1.215 &     70.58 &    30277 \\
(2) &     \palsgd &       32 &             4 &     1.397 &      67.31 &    1.257 &     69.68 &    29066 \\
(3) &         \mbsgd &      128 &             1 &     1.237 &      70.63 &    1.220 &     70.07 &    26772 \\
(4) &         \mbsgd &       32 &             1 &     1.339 &      68.53 &    1.231 &     70.13 &    30706 \\
(5) &        \plsgd &      128 &             1 &     1.256 &      70.22 &    1.223 &     70.02 &    25850 \\
(6) &        \plsgd &       32 &             1 &     1.350 &      68.32 &    1.236 &     70.02 &    31468 \\
\bottomrule
\end{tabular}


==> results/res20cifar100/Arch_res20_Data_cifar100.tex <==
\begin{tabular}{llllllllll}
	\toprule
	{} & \textbf{Method} & $\mathbf{B}$ & $\mathbf{K}$ & $\mathbf{U}$ & \textbf{Train{\newline}Loss} & \textbf{Test{\newline}Loss} & \textbf{Train{\newline}Acc.} & \textbf{Test{\newline}Acc.} & \textbf{Time{\newline}(S)} \\
	\midrule
  (1) &\alsgd &      128 &              6 &             6 &     0.295 &    1.191 &      92.23 &     69.43 &     1285 \\
  (2) &\alsgd &      128 &              8 &             4 &     0.299 &    1.198 &      92.15 &     69.28 &     1325 \\
 (3) &\palsgd &      128 &             16 &             4 &     0.378 &    1.161 &      89.50 &     69.75 &     1154 \\
 (4) &\palsgd &      128 &              6 &             6 &     0.404 &    1.173 &      88.69 &     69.47 &     1085 \\
(5) &\mbsgd &     1024 &              4 &             1 &     0.464 &    1.212 &      86.46 &     67.04 &     1244 \\
(6) &\mbsgd &      128 &              4 &             1 &     0.360 &    1.111 &      89.93 &     69.73 &     1754 \\
(7) &\plsgd &     1024 &             16 &             1 &     0.373 &  
1.152 &      89.48 &     67.97 &     1198 \\
(8) &\plsgd &      128 &             16 &             1 &     0.379 &    1.099 &      89.29 &     69.67 &     1613 \\
\bottomrule
\end{tabular}


==> results/sqnetcifar100/Arch_squuezenet_Data_cifar100.tex <==
\begin{tabular}{llllllllll}
\toprule
{} & \textbf{Method} & $\mathbf{B}$ & $\mathbf{K}$ & $\mathbf{U}$ & \textbf{Train{\newline}Loss} & \textbf{Test{\newline}Loss} & \textbf{Train{\newline}Acc.} & \textbf{Test{\newline}Acc.} & \textbf{Time{\newline}(S)} \\
\midrule
(1) &      \alsgd &      128 &             16 &             4 &     0.037 &    1.549 &      \textbf{99.56} &     \textbf{70.17} &     \textbf{1263} \\
(2) &     \palsgd &      128 &             16 &             4 &     0.070 &    1.504 &      98.79 &     \textbf{69.97} &     \textbf{1071} \\
(3) &         \mbsgd &     1024 &             16 &             1 &     0.043 &    1.294 &      99.60 &     68.30 &     1584 \\
(4) &         \mbsgd &      128 &             16 &             1 &     0.049 &    1.178 &      99.29 &     70.06 &     2134 \\
(5) &        \plsgd &     1024 &             16 &             1 &     0.061 &    1.259 &      99.25 &     68.46 &     1209 \\
(6) &        \plsgd &      128 &             16 &             1 &     0.062 &    1.207 &      99.00 &     69.38 &     1857 \\
\bottomrule
\end{tabular}


==> texts/asyn.tex <==
Consider a system that performs \palsgd with three workers $\mathcal{Q}=\{q_1,q_2,q_3\}$ in reference to Algorithm \ref{alg:algo}. The averaging processes on the three workers are denoted by $a^{q_1}$, $a^{q_2}$, and $a^{q_3}$, respectively. Suppose that the workers have a single updater process each: $u^{q_1}$, $u^{q_2}$, and $u^{q_3}$, respectively. Following the post local SGD scheme, the synchronization frequency--the number of local SGD updates--before the $1^{st}$ synchronization round (i.e. after the $0^{th}$ synchronization round) would be $K_0=1$. 

Now, consider the real-time scale and suppose that each of the processes on each of the workers started their operations, i.e. the updater processes take step of line \ref{line:initupdate} and the averaging processes take step of line \ref{line:initaverage}, at time $t=0$. Now, suppose that the averaging processes $a^{q_1}$, $a^{q_2}$, and $a^{q_3}$ take the steps to go past line \ref{line:checkupdate} to reach the synchronization step at line \ref{line:synchronize} at real-time points  $t_1,t_2,t_3>0$ s.t. $t_1<t_2<t_3$. Thus, the processes $a^{q_1}$ waits for $a^{q_2}$ and both of them wait for the process $a^{q_3}$ to perform the all-reduce averaging synchronization among the workers $q\in\mathcal{Q}$. Clearly, when they return to line \ref{line:checkupdate} for the $2^{nd}$ averaging round, it is likely that the three workers would have seen different number of updates by their updater processes $u^{q_1}$, $u^{q_2}$, and $u^{q_3}$ locally: the faster updater whose corresponding averaging process had to wait for others, possibly would have submitted a larger number of updates. We assume the delay bounds in Assumption \ref{as:delays}. This illustrates that the total number of synchronization rounds in the proposed asynchronous model is determined by the slowest updating worker. Thus, intuitively by design, the total number of synchronization rounds, and therefore the communication cost, in \alsgd and \palsgd is lower than that of \plsgd for the same sample budget. 
